Measuring Time with Minimal Clocks

Being able to measure time, whether directly or indirectly, is a significant advantage for an organism. It allows for the timely reaction to regular or predicted events, reducing the pressure for fast processing of sensory input. Thus, clocks are ubiquitous in biology. In the present paper, we consider minimal abstract pure clocks in different configurations and investigate their characteristic dynamics. We are especially interested in optimally time-resolving clocks. Among these, we find fundamentally diametral clock characteristics, such as oscillatory behavior for purely local time measurement or decay-based clocks measuring time periods of a scale global to the problem. We include also sets of independent clocks ("clock bags"), sequential cascades of clocks and composite clocks with controlled dependency. Clock cascades show a "condensation effect" and the composite clock shows various regimes of markedly different dynamics.

==> data/robu.dragged_counter_tradeoff.tex <==
\begin{tikzpicture}
\begin{axis}[
    xlabel=Information Flow Constraint,
    ylabel=Mutual Information,
    xmin=0, xmax=1,
    ymin=1.4,ymax=2
    % ymin=1.5,ymax=2
]

\addplot [] table[x index=0, y index=1] 
    {data/robu.drag_n9_mi_condmi_a.dat};
\addplot [] table[x index=0, y index=1] 
    {data/robu.drag_n9_mi_condmi_b.dat};
\addplot [] table[x index=0, y index=1] 
    {data/robu.drag_n9_mi_condmi_c.dat};
\end{axis}
\end{tikzpicture}





	

==> figs/robu.parameter_cloud.tex <==
\begin{tikzpicture}
\begin{axis}[axis on top,
  xmin=0,xmax=1,ymin=0,ymax=2,
%   colorbar,
%   colormap/bluered,
  xlabel=Information Flow,
  ylabel=Mutual Information,
  x=6.54cm,y=4.38cm/2
%   x=5cm,y=4cm/2
]
\addplot graphics [xmin=0,xmax=1,ymin=0,ymax=2]
  {figs/robu.parameter_cloud_n9_bw.png};
\end{axis}
\end{tikzpicture}
